Trusted Multi-view Learning for Long-tailed Classification

Class imbalance has been extensively studied in single-view scenarios; however, addressing this challenge in multi-view contexts remains an open problem, with even scarcer research focusing on trustworthy solutions. In this paper, we tackle a particularly challenging class imbalance problem in multi-view scenarios: long-tailed classification. We propose TMLC, a Trusted Multi-view Long-tailed Classification framework, which makes contributions on two critical aspects: opinion aggregation and pseudo-data generation. Specifically, inspired by Social Identity Theory, we design a group consensus opinion aggregation mechanism that guides decision making toward the direction favored by the majority of the group. In terms of pseudo-data generation, we introduce a novel distance metric to adapt SMOTE for multi-view scenarios and develop an uncertainty-guided data generation module that produces high-quality pseudo-data, effectively mitigating the adverse effects of class imbalance. Extensive experiments on long-tailed multi-view datasets demonstrate that our model is capable of achieving superior performance. The code is released at https://github.com/cncq-tang/TMLC.

==> sec/0_abstract.tex <==
\begin{abstract}
Class imbalance has been extensively studied in single-view scenarios; however, addressing this challenge in multi-view contexts remains an open problem, with even scarcer research focusing on trustworthy solutions. In this paper, we tackle a particularly challenging class imbalance problem in multi-view scenarios: long-tailed classification. We propose TMLC, a Trusted Multi-view Long-tailed Classification framework, which makes contributions on two critical aspects: opinion aggregation and pseudo-data generation. Specifically, inspired by Social Identity Theory, we design a group consensus opinion aggregation mechanism that guides decision-making toward the direction favored by the majority of the group. In terms of pseudo-data generation, we introduce a novel distance metric to adapt SMOTE for multi-view scenarios and develop an uncertainty-guided data generation module that produces high-quality pseudo-data, effectively mitigating the adverse effects of class imbalance. Extensive experiments on long-tailed multi-view datasets demonstrate that our model is capable of achieving superior performance.
\end{abstract}

==> sec/1_introction.tex <==
\section{Introduction}
\label{sec:intro}

Class imbalance refers to a situation in which the distribution of classes in a dataset is non-uniform, characterized by significant or even extreme disparities~\cite{kang2020exploring,menon2020long}. This phenomenon, widely observed in real-world scenarios such as fraud detection~\cite{zhang2021fraudre} and medical image analysis~\cite{ju2021relational}, often arises due to limitations or biases in the data collection process. In the machine learning community, class imbalance is recognized as a critical research challenge, as models trained on imbalanced data tend to favor the majority class while neglecting the minority class~\cite{wang2020long,cao2019learning,tan2020equalization}. This can result in suboptimal performance, particularly for those predictions where accurate classification of the minority class is essential. 

Research on class imbalance mainly follows three technical routes: re-sampling~\cite{chawla2002smote,estabrooks2004multiple,liu2008exploratory}, cost-sensitive learning~\cite{elkan2001foundations,hsieh2021droploss}, and data augmentation~\cite{chu2020feature,liu2020deep,wang2017effectiveness}. Re-sampling methods aim to balance class distributions by either over-sampling minority classes or under-sampling majority classes, with two well-known techniques being SMOTE~\cite{chawla2002smote} and Tomek Links~\cite{4309452}. In contrast to re-sampling, which focuses on data generation, cost-sensitive learning addresses class imbalance by assigning higher misclassification costs to minority classes through weighted loss functions~\cite{lin2017focal,cui2019class,ren2020balanced} or specialized algorithms~\cite{cao2019learning,khan2019striking}. This approach offers flexibility but often requires careful tuning of cost parameters. Data augmentation, on the other hand, highlights the diversity of minority class samples using techniques such as generative models~\cite{ji2024tltscore} or feature-space transformations~\cite{chu2020feature,wang2017learning}. It is worth noting that, although both re-sampling and data augmentation methods essentially fall under pseudo-data generation approaches, they differ significantly in their mechanisms: re-sampling focuses on adjusting data distribution, whereas data augmentation emphasizes enriching data diversity.

The aforementioned studies on class imbalance have been conducted in single-view scenarios, where decision-making relies on a single modality of data. However, real-world applications often involve multi-view scenarios~\cite{lee2023mvfs,fan2022mv}, in which multiple data sources are available for analysis. For instance, in medical diagnosis~\cite{perrin2009multimodal,sui2018multimodal}, multi-view data may include X-ray images, MRI scans, and other modalities, each offering unique and complementary insights into patient conditions. To the best of our knowledge, addressing class imbalance in such multi-view settings remains an open and under-explored challenge, which demands innovative solutions and deeper investigation.

In this paper, we address a particularly challenging class imbalance problem—long-tailed distribution class imbalance—in multi-view scenarios. \textit{We aim to answer two critical questions: (1) How to tackle the challenge of multi-view long-tailed classification, and (2) how to ensure reliable decision-making?} To this end, we propose TMLC, a Trusted Multi-View Long-Tailed Classification Framework , as shown in \cref{fig:TMLC}. TMLC is designed to achieve trustworthy classification for multi-view long-tailed data by leveraging a deep evidence learning-inspired paradigm~\cite{sensoy2018evidential} and adopting a oversampling-based scheme. Specifically, we make significant advancements in opinion aggregation and pseudo-data generation, which respectively enhance the reliability of the trustworthy framework and improve the effectiveness of the oversampling process. The main contributions of this work are as follows:

\begin{itemize}
    \item Motivated from Social Identity Theory~\cite{hogg2016social}, we design a group consensus opinion aggregation mechanism that guides decision-making toward the direction favored by the majority of the group, thereby preventing negative individual opinions from dominating the final outcome.
    \item To address the limitation of SMOTE, which cannot be directly applied to multi-view settings, we introduce a novel distance metric based on joint subjective evidence and propose an uncertainty-based sample generation scheme that enables the production of high-quality pseudo-data.
    \item Extensive experiments on long-tailed multi-view datasets demonstrated that TMLC outperforms serveral state-of-art baselines.
\end{itemize}


==> sec/2_related.tex <==
\section{Related Work}

% \textbf{Long-tailed learning.} Traditional long-tailed learning methods include re-sampling, cost-sensitive learning and data augmentation. Class re-balancing is a mainstream paradigm in long-tailed learning, including Re-sampling~\cite{chawla2002smote},~\cite{estabrooks2004multiple},~\cite{liu2008exploratory}, cost-sensitive learning~\cite{hsieh2021droploss},~\cite{chen2023cost},~\cite{zhao2018adaptive} and logit adjustment~\cite{menon2020long},~\cite{wu2021adversarial},~\cite{zhang2021distribution}. 


% methods balance class distribution by modifying the class sample distribution in each mini-batch. DCL~\cite{wang2019dynamic} has developed a novel curriculum strategy for dynamically sampling data to achieve class re-balancing. Class-sensitive learning aims to counteract class imbalance by adjusting the training loss for different classes. Focal Loss~\cite{lin2017focal} and cost-sensitive learning~\cite{chen2023cost},~\cite{zhao2018adaptive} assign different weights to different classes, which allow the model to focus more on minority class samples. Logit adjustment~\cite{menon2020long},~\cite{wu2021adversarial},~\cite{zhang2021distribution} correct class imbalance by modifying the model’s prediction logits.

\textbf{Long-tailed Learning.} Traditional long-tailed learning methods include re-sampling~\cite{han2005borderline,liu2008exploratory}, cost-sensitive learning~\cite{cui2019class,cao2019learning,wang2021adaptive} and data augmentation~\cite{chu2020feature,kim2020m2m,yin2019feature}. As one of the most widely used techniques, Re-sampling rebalances classes by adjusting the number of samples per class. SMOTE~\cite{chawla2002smote} enhances the representation of minority classes by generating synthetic samples. Decoupling~\cite{kang2019decoupling} identifies effective sampling strategies for standard model training. DCL~\cite{wang2019dynamic} and LOCE~\cite{feng2021exploring} propose adaptive sampling strategies. Balanced Meta-Softmax~\cite{ren2020balanced} employs meta-learning to estimate optimal sampling rates for different classes. SimCal~\cite{wang2020devil} uses a novel two-level class-balanced sampling strategy that combines image-level and instance-level. However, these methods do not fully explore the uncertainty of samples during the sampling phase.

\noindent \textbf{Uncertainty-induced Trusted Learning.} Inspired by evidential deep learning~\cite{sensoy2018evidential}, which serves as a prominent paradigm for uncertainty estimation, Trusted Multi-view Classification (TMC) has recently gained particular attention. TMC leverages the Dirichlet distribution to model class probabilities and integrates Dempster-Shafer theory to achieve reliable classification results~\cite{han2022trusted}. Based on TMC, numerous extensions have been proposed to tackle specific challenges, involving conflicting opinion aggregation  ~\cite{liu2022trusted, xu2024reliable}, noisy labels~\cite{xu2024trusted}, semantic ambiguity~\cite{liu2024dynamic}, etc. Recent advancements in trusted learning have expanded its research to areas such as semi-supervised learning, multimodal fusion, and open-world learning, as detailed in works~\cite{zhou2023rtmc, wang2024trusted, du2023bridging, zhou2023calm}.

==> sec/3_method.tex <==
\section{Methodology}

In this section, we first provide the problem definition and theoretical foundation on evidential deep learning. Subsequently, we detail our key contributions, including the group consensus opinion aggregation mechanism and the uncertainty-based sample generation scheme.

%\begin{figure*}[t]
%  \centering
%   \includegraphics[width=0.8\linewidth]{img/TMLC.pdf}
%   \caption{Illustration of TMLC. Assuming that the opinions from the first $V-1$ views have been aggregated, we now focus on combining the resulting joint opinion $\boldsymbol{e}^{\Diamond(V-1)}$ with the opinion $\boldsymbol{e}^{V}$ from the $V$-th view. In this process, a larger weight is assigned to $\boldsymbol{e}^{\Diamond(V-1)}$ which respresents the group joint opinion, while a smaller weight is assigned to the individual opinion $\boldsymbol{e}^{V}$. This strategy prioritizes the consensus of the majority of views, thereby enhancing the reliability of the decision-making process. Subsequently, we propose an uncertainty-based sample generation scheme to ensure the production of reliable pseudo-data for the minority class.}
%   \label{fig:TMLC}
%\end{figure*}

\begin{figure*}[t]
  \centering
   \includegraphics[width=0.8\linewidth]{img/TMLC.pdf}
   \caption{Illustration of TMLC. Assuming that the opinions from the first $V-1$ views have been aggregated, we now focus on combining the resulting joint opinion $\boldsymbol{e}^{\Diamond(V-1)}$ with the opinion $\boldsymbol{e}^{V}$ from the $V$-th view. In this process, a larger weight is assigned to $\boldsymbol{e}^{\Diamond(V-1)}$ which respresents the group joint opinion, while a smaller weight is assigned to the individual opinion $\boldsymbol{e}^{V}$. Subsequently, we propose an uncertainty-based sample generation scheme to ensure the production of reliable pseudo-data for the minority class.}
   \label{fig:TMLC}
\end{figure*}

\subsection{Problem Definition and Preliminaries}

\subsubsection{Problem Definition}

A long-tailed multi-view dataset typically contains an imbalanced training set and a balanced test set. For a $K$ classification problem, we define the multi-view data as $\{\boldsymbol{X}^{v}\}^V_{v=1}$ and the corresponding ground-truth labels as $\{\boldsymbol{\mathrm{y}}_{n} \}_{n=1}^{N}$ with $V$ views and $N$ samples, where $\boldsymbol{X}^{v} =[\boldsymbol{x}^v_1,\boldsymbol{x}^v_2,\cdots,\boldsymbol{x}^v_N] \in \mathbb{R}^{d_v\times N}$ represents the $v$-th view data with $d_v$ dimension. For each view data $\boldsymbol{X}^{v}$, the distribution of classes is highly imbalanced, with tail classes having significantly fewer samples compared to head classes. The goal of TMLC is to address the challenges caused by imbalanced class distributions.    

\subsubsection{Evidential Deep Learning}

Evidential Deep Learning (EDL) ~\cite{sensoy2018evidential} is a probabilistic framework to model prediction uncertainty by employing evidential priors and subjective logic ~\cite{josang2016subjective}. In the EDL framework, the evidences $\boldsymbol{e}^v = [e^v_1,\cdots,e_K^v]$ for the $v$-th are obtained using Deep Neural Networks (DNNs), where the Softmax layer is replaced by a ReLU activation function.

Subjective logic provides a technical approach to associate the evidence $\boldsymbol{e}^v = [e^v_1,\cdots,e_K^v]$ with the parameters of the Dirichlet distribution $\boldsymbol{\alpha}^v = [\alpha_1^v,\cdots,\alpha_K^v]$. Specifically, each parameter $\alpha^v_k$ of the Dirichlet distribution is derived from $e^v_k$ as $\alpha^v_k = e^v_k + 1$. The belief mass $b^v_k$ and the uncertainty $u^v$ are then calculated as follows:
\begin{equation} 
b_k^v = \frac{e_k^v}{S^v} = \frac{\alpha_k^v - 1}{S^v} \quad \text{and} \quad u^v = \frac{K}{S^v},
\label{eq01}
\end{equation}
where $S^v = \sum\nolimits_{k=1}^{K} (e_k^v + 1) = \sum\nolimits_{k=1}^{K} \alpha^v_k$ denotes the Dirichlet strength. The projection probability is calculated by
\begin{equation}
    P_k^v = b_k^v + a_k^v u^v.
    \label{eq01_r1}
\end{equation}

From \cref{eq01}, we can obtain an ordered triplet $\omega=(\boldsymbol{b},u,\boldsymbol{a})$ that reflects the multinomial opinion of an instance $\boldsymbol{x}^v_n$. Since the Dirichlet distribution parameter $\boldsymbol{a}$ is derived from the belief mass $\boldsymbol{b}$, a simplified representation of the multinomial opinion can be expressed as $\mathcal{M}=\{\boldsymbol{b},u\}$. Once multinomial opinions from multiple views are derived, designing an efficient opinion aggregation strategy becomes crucial for achieving trusted decision-making.  


\subsection{Group Consensus Opinion Aggregation}

Social Identity Theory posits that individuals tend to value shared group opinions over personal viewpoints, which helps avoid conflict and fosters stable social environments \cite{hogg2016social}. Inspired by this theory, we argue that in a trusted decision-making process, partial aggregated group opinions should be prioritized over individual opinions. To this end, we propose a novel opinion aggregation strategy, termed Group Consensus Opinion Aggregation, which is detailed below.
 
%According to the above, we can get the opinion combination of $V$ views $\{ \mathcal{M}^v=(\boldsymbol{b}^v,u^v)\}_{v=1}^V$. Therefore, in this section, we focus on multi-view fusion based on view-specific opinions. ECML~\cite{xu2024reliable} has been proposed, which provides a novel opinion fusion framework that aims to reduce the impact of conflicting noise of multi-view data. However, in the opinion fusion stage between any two views, simply averaging the evidence of the two opinions to obtain the fused opinion is not completely reasonable in our opinion. 
%
%Specifically, during the initial stage of opinion fusion, the input opinions are derived from two distinct views. In the absence of any prior knowledge indicating that one view is more important than the other, we assume both views are equally significant and therefore fuse their opinions by averaging, which assigns each view a weight of $1/2$. However, because the fused opinion represents aggregate information from multiple views, it is inappropriate in subsequent fusion stages to treat this collective opinion as having the same importance as that of the individual views. Inspired by social psychology \textcolor{blue}{ref}, which suggests that in a fair decision-making process the collective decision of the majority should be prioritized over individual opinion, we propose a novel fusion mechanism called group consensus opinion aggregation in Definition 1, which is based on consensus among group opinions for multi-view evidence fusion.

\textbf{Definition 1.} \textbf{\textit{Group Consensus Opinion Aggregation.}} Without loss of generality, each view is assumed to be equally important. For $V$ opinions $\{\mathcal{M}^1,\mathcal{M}^2,\cdots,\mathcal{M}^V\}$, we aggregate them via

\begin{equation}
    \mathcal{M}^{\Diamond(V)} = \underbrace{\underbrace{\underbrace{\mathcal{M}^1 \oplus \mathcal{M}^2}_{\mathcal{M}^{\Diamond(2)}} \oplus \mathcal{M}^3}_{\mathcal{M}^{\Diamond(3)}} \oplus \dots \oplus \mathcal{M}^{V-1}}_{\mathcal{M}^{\Diamond(V-1)}} \oplus \mathcal{M}^V,
    \label{eq02}
\end{equation}
where $\mathcal{M}^{\Diamond(V)} = \{\boldsymbol{b}^{\Diamond(V)},u^{\Diamond(V)}\}$. Regarding the calculation of $\boldsymbol{b}^{\Diamond(V)}$ and $u^{\Diamond(V)}$, we present the aggregation process corresponding to their $k$-th components:
\begin{equation}
	\begin{aligned}
    b_k^{\Diamond(V)} &= \frac{e_k^{\Diamond(V)}}{S^{\Diamond(V)}}=\frac{\gamma^{\Diamond(V-1)} e_k^{\Diamond(V-1)} +\gamma^V e_k^V}{\gamma^{\Diamond(V-1)} S^{\Diamond(V-1)} + \gamma^V S^V},\\
    \end{aligned}
    \label{eq02_1}
\end{equation}
and 
\begin{equation}
	\begin{aligned}
	u^{\Diamond(V)}&=\frac{K}{\sum_{k=1}^{K}(e_k^{\Diamond(V)}+1)}\\
	&=\frac{K}{\sum_{k=1}^{K}(\gamma^{\Diamond(V-1)} e_k^{\Diamond(V-1)}+ \gamma^V e_k^V+1)},\\
	\end{aligned}
	\label{eq02_2}
\end{equation}
with $\gamma^{\Diamond(V-1)}$ and $\gamma^V$ being
\begin{equation}
    \gamma^{\Diamond(V-1)}=\frac{V-1}{V},\;\; \gamma^V=\frac{1}{V}.
    \label{eq05}
\end{equation}

From \cref{eq02_1} to \cref{eq05}, we see that the aggregated evidence $e_k^{\Diamond(V-1)}$ for the first $V-1$ views is assigned with a large weight $\gamma^{\Diamond(V-1)}$, whereas the evidence $e^V_k$ to be aggregated is assigned with a small weight $\gamma^V$. This indicates that, in the opinion aggregation process, the aggregated group opinion will play a dominant role. The further calculation results for \cref{eq02_1} and \cref{eq02_2} are given by
%\begin{equation}
%    b_k^{\Diamond(V)} = \frac{\gamma^{\Diamond(V-1)}b_k^{\Diamond(V-1)} u^V + b_k^V u^{\Diamond(V-1)}}{\gamma^V u^{\Diamond(V-1)}+\gamma^{\Diamond(V-1)}u^V},
%    \label{eq03}
%\end{equation}
\begin{equation}
    b_k^{\Diamond(V)}=\frac{\gamma^{\Diamond(V-1)} b_k^{\Diamond(V-1)}u^V + \gamma^V b_k^V u^{\Diamond(V-1)}}{\gamma^V u^{\Diamond(V-1)}+ \gamma^{\Diamond(V-1)}u^V}
    \label{eq03}
\end{equation}
and 
\begin{equation}
    u^{\Diamond(V)} = \frac{u^{\Diamond(V-1)} u^V}{\gamma^V u^{\Diamond(V-1)}+\gamma^{\Diamond(V-1)}u^V}
    \label{eq04}
\end{equation}
The detailed derivation for the above equations and its effectiveness can be found in the supplementary material.

%Assuming that the importance of $V$ views is equal, the importance of the fused opinion is the superposition of the importance of the fused views. Given joint opinions of the $M(M=1,\cdots,V-1)$ views $\mathcal{M}^{\Diamond(M)}=\{\boldsymbol{b}^{\Diamond(M)},u^{\Diamond(M)}\}$ and $v$-th view opinion $\mathcal{M}^v=\{\boldsymbol{b}^v,u^v\}$ under the same sample, the fused opinion can be calculated by the following formula:
%\begin{equation}
%    \mathcal{M}^{\Diamond(M+1)}=\mathcal{M}^{\Diamond(M)} \oplus \mathcal{M}^v=\left(\boldsymbol{b}^{\Diamond(M+1)},u^{\Diamond(M+1)} \right) 
%\end{equation}
%\begin{equation}
%    b_k^{\Diamond(M+1)} = \frac{\gamma^{\Diamond(M)}b_k^{\Diamond(M)} u^v + b_k^v u^{\Diamond(M)}}{\gamma^v u^{\Diamond(M)}+\gamma^{\Diamond(M)}u^v}
%\end{equation}
%\begin{equation}
%    u^{\Diamond(M+1)} = \frac{u^{\Diamond(M)} u^v}{\gamma^v u^{\Diamond(M)}+\gamma^{\Diamond(M)}u^v}
%\end{equation}
%\begin{equation}
%    \gamma^{\Diamond(M)}=\frac{M}{M+1},
%    \gamma^v=\frac{1}{M+1}
%\end{equation}

Our proposed aggregation strategy ensures that the group joint opinion is given higher priority than the individual subjective opinion. When dealing with conflicting opinions, our scheme tends to favor the group consensus opinion, thereby enhancing the realibity of decision-making.
%
%Following Definition 1, we can fusion the final joint opinions:
%\begin{equation}
%    \mathcal{M} = \mathcal{M}^{\Diamond(1)} \oplus \mathcal{M}^2 \oplus \cdots \oplus \mathcal{M}^V
%\end{equation}
%where $\mathcal{M}^{\Diamond(1)}=\mathcal{M}^1$ in the first opinion fusion. Based on the aforementioned fusion rules, we derive the final multi-view joint opinion, which yields both the joint class probabilities and overall uncertainty that gives as prior knowledge for subsequent class balancing methods.

\subsection{Uncertainty-based Sample Generation}

A common strategy for addressing the challenge of class imbalance is to generate new samples for the minority class to construct a balanced dataset. Among various techniques, the SMOTE method~\cite{chawla2002smote} is a well-established and straightforward approach that yields new samples by linearly interpolating between minority class samples and their nearest neighbors. While traditional SMOTE is effective in single-view scenarios, it is not directly applicable to multi-view settings. The primary challenge lies in the fact that SMOTE relies on neighbor analysis based on Euclidean distance calculations, which may yield inconsistent results across different views due to the inherent diversity among them. Specifically, the neighbor relationships identified in each view can differ significantly, potentially leading to conflicts in the synthetic samples generated from different views.

%The SMOTE method needs to perform a neighbor analysis before generating a new sample and determine its neighbors by distance (such as Euclidean distance). However, traditional distance measurement methods are not directly applicable to distance calculation between multi-view sample data. 

To overcome the aforementioned drawback, we attempt to introduce a distance metric to adapt SMOTE for multi-view scenarios. We build upon a natural premise: samples belonging to the same class exhibit consistency in their subjective opinions. Consequently, it is reasonable to infer that samples from the same category should also show similar evidence distributions. Based on this assumption, we develop a novel distance metric based on joint evidences. 

%In Section 3.3, we obtained the all views joint opinions $\mathcal{M}=\{\boldsymbol{b}, u\}$, according to Eq.\ref{eq.4}, the corresponding joint evidence from multiple views is induced as:
%\begin{equation}
%    S=\frac{K}{u},e_k=b_k\times S
%\end{equation}
%It is assumed that samples of the same category should generally show consistency in their subjective opinions on the same category, and the comprehensive evidence distributions of samples of the same category are similar. Therefore, we introduce a new distance metric, called the subjective evidence-based distance metric in Definition 2, which is built based on the joint evidence.

\textbf{Definition 2.} \textbf{\textit{Distance measures based on joint subjective evidence.}} Given any two samples $\{\boldsymbol{x}_i^v\}_{v=1}^V$ and $\{\boldsymbol{x}_j^v\}_{v=1}^V$, along with their corresponding joint opinions $\boldsymbol{e}_i$, $\boldsymbol{e}_j$, the distance between these two samples is defined as:
\begin{equation}
    D(\boldsymbol{x}_i,\boldsymbol{x}_j)=\sqrt{(e_{i1}-e_{j1})^2+\cdots+(e_{iK}-e_{jK})^2}.
    \label{eq06}
\end{equation}
In \cref{eq06}, a smaller distance indicates a higher similarity between samples.

Apart from the limitation that the traditional SMOTE method cannot be applied to multi-view settings, another problem is that during the pseudo-data generation process, the weights for combining the center sample with its neighors are randomly selected, which may result in undesirable pseudo samples. To address this, we design an uncertainty-based sample generation scheme that ensures neighbors with low-uncertainty opinion are assigned with higher weights, thereby facilitating the generation of high-quality pseudo-samples. In the following, we present the details of our designed scheme.

For a minority class, we randomly select a data sample $\{\boldsymbol{x}_{\text{c}}^v\}_{v=1}^V$ as the center. The $R$ samples with the shortest distances to the center sample, calculated using \cref{eq06}, are identified as its neighbors and denoted as $\{\boldsymbol{x}_1^v, \boldsymbol{x}_2^v, \dots, \boldsymbol{x}_R^v\}_{v=1}^V$. For the $v$-th view, the new pseudo sample is generated by
\begin{equation}
    \boldsymbol{x}_{new}^v =w_0^v\boldsymbol{x}_\text{c}^v+w_1^v\boldsymbol{x}_1^v+\cdots+w_R^v\boldsymbol{x}_R^v,
    \label{eq07}
\end{equation}
where $\sum_{r=0}^R w_r^v=1$ and $w_r^v\ge 0$. We expect that the weight $w^v_r$ to be assigned a high value if the aggregated opinion between the corresponding neighbor $\boldsymbol{x}^v_r$ and the center sample $\boldsymbol{x}^v_c$ exhibits low uncertainty, indicating that the relationship between this neighbor and the center sample is highly reliable. To achieve this objective, we begin with integrating the evidence of $\boldsymbol{x}^v_c$ with that of $\boldsymbol{x}^v_r$
\begin{equation}
    \boldsymbol{e}_{cr}^v = \frac{1}{2}\boldsymbol{e}_\text{c}^v+\frac{1}{2}\boldsymbol{e}_r^v,\;\; r=0,1,\cdots,R
    \label{eq08}
\end{equation}   
With the integrated evidence in \cref{eq08} and recalling \cref{eq01}, we can obtain the corresponding opinions and projection probabilities for the neighbors, denoted as $\{\boldsymbol{b}_{cr}^v,u_{cr}^v\}_{r=0}^R$ and $\{\boldsymbol{P}^v_{cr}\}^R_{r=0}$, respectively. 

Here, we treat the projection probalibity as the prediction probability. This leads to a straightforward approach for aligning the distribution of the generated pseudo-samples with the true distribution, typically measured by cross-entropy. However, directly using cross entropy can not reflect the reliability of the generated samples. Thus, we introduce the influence of uncertainty and propose a novel criterion, termed Uncertainty Entropy. 

\textbf{Definition 3.} \textbf{\textit{Uncertainty Entropy.}} Given an opinion $\mathcal{M}=\{\boldsymbol{b}, u\}$ and the true label $\boldsymbol{y}$, the uncertainty entropy is defined as:
\begin{equation}
    H = -\text{exp}(u)\sum_{k=1}^K y_k \text{log}(b_k+ua_k),
    \label{eq09}
\end{equation}
where $\text{exp}(u)$ is the penalty coefficient. If the uncertainty $u=0$, then $\text{exp}(u)=1$, and the uncertainty has no effect on the entropy. Conversely, as the uncertainty $u$ increases, the entropy value also increases, indicating a greater discrepancy between the predicted classification and the true class.

With uncertainty entropy, we further present the following formulation for calculating $w^v_r$
\begin{equation}
    w_r^v = \frac{\mathcal{F}(H_{cr}^v)}{\mathcal{F}(H_c^v)+\sum_{r=1}^R\mathcal{F}(H_{cr}^v)}, \; r=0,1,\cdots,R  
    \label{eq10}
\end{equation}
where $\mathcal{F}(\cdot)$ is a monotonically decreasing function. If the uncertainty is low, from the above discussion, we know that the uncertainty entropy is small. Due to the monotonically decreasing property of $\mathcal{F}(\cdot)$, $\mathcal{F}(H_{cr}^v)$ will be assigned a large value. This implies that our scheme is capable of ensuring that neighbors with low-uncertainty opinions are assigned higher weights. In this paper, we use $\mathcal{F}(x)=x^{-1}$.

\subsection{Loss Function}

%In this subsection, we will introduce how to train DNN to obtain multi-view joint opinions. The subsequent pseudo-samples are mainly generated based on the trained DNN, without the need for additional loss functions. We transform the network into an evidential DNN by replacing the softmax layer of the traditional DNN with a ReLU activation layer and treating the non-negative output of this layer as evidence. In this way, we can obtain the parameters of the Dirichlet distribution.

In this subsection, we introduce the loss function for taining our model. We first employ an adjusted cross-entropy loss function to ensure that all views generate appropriate non-negative view-specific evidence for classification:
\begin{equation} 
    \begin{aligned}  
        L_{ace}(\boldsymbol{\alpha}_n) &= \int \left[ \sum_{k=1}^{K}-y_{nk}\log p_{nk} \right] \frac{\Pi_{k=1}^K p_{nk}^{\alpha_{nk}-1}}{B(\alpha_n)}d_{P_n}\\   
        &=\sum_{k=1}^{K} y_{nk}(\psi(S_n) - \psi(\alpha_{nk}),
    \end{aligned}  
\end{equation}
where $\psi(\cdot)$ is the digamma function. 

Additionally, to ensure that incorrect classes in each sample produce lower evidence, we incorporate an extra KL divergence term into the loss function

\begin{equation}
    \begin{aligned} 
        L_{KL}(\boldsymbol{\alpha}_n) &= KL \left[D(p_n|\tilde{\alpha}_n)||D(p_n|1)\right]\\
        &= \log(\frac{\Gamma(\sum_{k=1}^{K} \tilde{\alpha}_{nk})}{\Gamma(K)\Pi^K_{k=1}\Gamma(\tilde{\alpha}_{nk})})\\
        &+\sum_{k=1}^{K}(\tilde{\alpha}_{nk}-1) \left[\psi(\tilde{\alpha}_{nk}) - \psi(\sum_{j=1}^{K}\tilde{\alpha}_{nj})\right],
    \end{aligned}  
\end{equation}
where $D(p_n|1)$ is the uniform Dirichlet distribution, $\tilde{\boldsymbol{\alpha}}_{n} = \boldsymbol{y}_n + (1-\boldsymbol{y}_n)\odot \boldsymbol{\alpha}_n$ is the Dirichlet parameters that reduces the incorrect classes to zero for the $n$-th instance, and $\Gamma(\cdot)$ is the gamma function. Therefore, given the Dirichlet distribution with parameter $\boldsymbol{\alpha}_n$ for the $n$-th instance, the loss is:

\begin{equation}
    L_{acc}(\boldsymbol{\alpha}_n) = L_{ace}(\boldsymbol{\alpha}_n) + \lambda_t L_KL(\boldsymbol{\alpha}_n)
\end{equation}
where $\lambda_t\in[0,1]$ is a balance factor with $t$ being the current training epoch index. The implementation procedures are summarized in Algorithm \ref{algorithm}.

\begin{algorithm}
    \caption{Implementation pseudocode of TMLC}
    \begin{algorithmic}
        \item[]\hspace*{-\algorithmicindent}\textbf{Input:} Multi-view dataset: $\{\boldsymbol{X}^v, \boldsymbol{y}\}_{v=1}^V$
        % \item[]\hspace*{-\algorithmicindent}\textbf{Parameter:} Hyper-parameter: $R=5$
         \item[]\hspace*{-\algorithmicindent}/---Train---/
         \item[]\hspace*{-\algorithmicindent}\textbf{Output:} Network's parameters.
        \STATE 01: \textbf{while} not converged \textbf{do}
        % \STATE 02: \quad Initialize common features $\boldsymbol{c}$.
        \STATE 02: \quad \textbf{for} $v=1:V$  \textbf{do}
        \STATE 03: \qquad $\textbf{e}^v$ $\leftarrow$ evidential network output.
        \STATE 04: \qquad Calculate opinion $\mathcal{M}^v$ by Eq. (1).
        \STATE 05: \quad \textbf{end for}
        \STATE 06: \quad Calculate joint opinion $\mathcal{M}^{\Diamond(V)}$ by Eq. (3).
        \STATE 07: \quad Calculate joint evidence $\boldsymbol{e}$ by Eq. (1).
        \STATE 08: \quad Calculate the joint distribution $\boldsymbol{\alpha}=\boldsymbol{e}+1$. 
        \STATE 09: \quad Calculate the overall loss $\mathcal{L}$ by Eq. (16).
        \STATE 10: \quad Update the networks by gradient descent by $\mathcal{L}$.
        \STATE 11: \textbf{end while}
        \STATE 12: Initialize pseudo-data set $\{\}$.
        \STATE 13: \textbf{while} minority class $k$-th not balanced \textbf{do}
        \STATE 14: \quad  Randomly select a center sample $\{\boldsymbol{x}_{\text{c}}^v\}_{v=1}^V$.
        \STATE 15: \quad Calculate multi-view neighbors by Eq. (9).
        \STATE 16: \quad \textbf{for} $v=1:V$  \textbf{do}
        \STATE 17: \qquad Generate pseudo date $\boldsymbol{x}_{new}^v$ by Eq. (10).
        \STATE 18: \quad \textbf{end while}
        \STATE 18: \quad Add $\left\{ \{\boldsymbol{x}_{new}^v\}_{v=1}^V,y_k=1\right\}$ to pseudo-data set.
        \STATE 19: \textbf{end for}
        \STATE 20: Add pseudo-data set to the training set.
        \STATE 21: Repeat training steps 01-11.
        \STATE 22: \textbf{return} networks parameters.
        \item[]\hspace*{-\algorithmicindent}/---Test---/
        \item[]\hspace*{-\algorithmicindent}\textbf{Output:}The final classification prediction and uncertainty. 
        \STATE 01: \textbf{for} $v=1:V$  \textbf{do}
        \STATE 02: \quad $\textbf{e}^v$ $\leftarrow$ evidential network output.
        \STATE 03: \quad Calculate opinion $\mathcal{M}^v$ by Eq. (1).
        \STATE 04: \textbf{end for}
        \STATE 05: Calculate joint opinion $\mathcal{M}^{\Diamond(V)}$ by Eq. (3).
        \STATE 06: \textbf{return} the decision $\boldsymbol{b}^{\Diamond(V)}$ and uncertainty $u^{\Diamond(V)}$.
    \end{algorithmic}
    \label{algorithm}
\end{algorithm}

==> sec/4_experiment.tex <==
\section{Experiment}

In this section, we compare the classification accuracy of TMLC with existing state-of-the-art methods and demonstrate its effectiveness. 

\subsection{Experimental Setup}
\textbf{Datasets.} \textbf{HandWritten}\footnotemark\footnotetext{https://archive.ics.uci.edu/ml/datasets/Multiple+Features} comprises 2000 instances of handwritten numerals ranging form ‘0’ to ‘9’, with 200 patterns per class. It is represented using six feature sets. \textbf{PIE}\footnotemark\footnotetext{http://www.cs.cmu.edu/afs/cs/project/PIE/MultiPie/MultiPie Home.html}  contains 680 instances belonging to 68 classes. We extract intensity, LBP, and Gabor as 3 views. \textbf{Caltech101}\footnotemark\footnotetext{http://www.vision.caltech.edu/Image Datasets/Caltech101} comprises 8677 images from 101 classes. We select 2386 samples from 20 classes, where each image has six features: Gabor, Wavelet Moments, CENTRIST, HOG, GIST, and LBP. \textbf{NUS-WIDE}\footnotemark\footnotetext{https://paperswithcode.com/dataset/nus-wide} consists of 269,648 images with 81 concepts. For the top 12 classes, we select 200 images from each class, with a total of 6 different views. \textbf{Scene15}\footnotemark\footnotetext{https://doi.org/10.6084/m9.figshare.7007177.v1} includes 4485 images from 15 indoor and outdoor scene categories. We extract three types of features GIST, PHOG, and LBP. \textbf{Animal}\footnotemark\footnotetext{http://attributes.kyb.tuebingen.mpg.de/} contains 37,322 images of 50 animal species with six features for each image. We select 11,673 samples contained 20 animal classes and four features for 4 views. \cref{table:dataset} shows the details of datasets.

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Size} & \textbf{$K$} & \textbf{Dimensionality} \\ \hline
HandWritten & 2000 & 10 & 240/76/216/47/64/6 \\ \hline
PIE & 680 & 68 & 484/256/279 \\ \hline
Caltech101 & 2386 & 20 & 48/40/254/1984/512/928 \\ \hline
NUS-WIDE & 2400 & 12 & 64/144/73/128/225/500 \\ \hline
Scene15 & 4485 & 15 & 20/59/40 \\ \hline
Animal & 11673 & 20 & 2689/2000/2001/2000 \\ \hline
\end{tabular}
\caption{Dataset summary.}
\label{table:dataset}
\end{table}

\textbf{Compared Methods.} The compared methods involve long-tail methods, trusted multi-view learning and other multi-view baselines. Specifically, 1) long-tail methods include: \textbf{TLC} (Trustworthy Long-tailed Classification)~\cite{li2022trustworthy} combines classification and uncertainty estimation in a multi-expert framework with dynamic expert engagement. \textbf{H2T} (Head-To-Tail)~\cite{li2024feature} augments tail classes by incorporating the diverse semantic information from head classes. 2) Trusted multi-view decision baselines include: \textbf{TMC} (Trusted Multi-view Classification)~\cite{han2022trusted} integrates different views at an evidence level using variational Dirichlet distribution and Dempster-Shafer theory. \textbf{ECML} (Evidential Conflictive Multi-view Learning)~\cite{xu2024reliable} puts forward a conflictive opinion aggregation model. 3) Multi-view classification baselines include: \textbf{DUA-Nets} (Dynamic Uncertainty-Aware Networks)~\cite{geng2021uncertainty} is an uncertainty aware method,that uses reversal networks to integrate intrinsic information from different views into a unified representation. \textbf{DCP} (Dual Contrastive Prediction)~\cite{lin2022dual} enables consistency learning and missing view recovery by using an information-theoretical framework. \textbf{UIMC} (Uncertainty for Incomplete Multi-View Classification)~\cite{xie2023exploring} models the uncertainty of missing views through distribution construction and sampling and employs an evidence-based fusion strategy for trustworthy integration of imputed views. \textbf{DMVLS} (Dynamic Multi-view Labeling Strategy)~\cite{wan2024decouple} leverages shared and specific information with two classifiers to prioritize labeling low-confidence samples.

\textbf{Implementation Details.} To generate a class-imbalanced training set and a class-balanced testing set, we conduct the following operations: (1) We randomly select 80\% of the samples for training and use the remaining 20\% for testing, thereby creating the standard training and test sets. (2) To further construct a long-tailed training set from the standard training set, we employ a widely adopted strategy~\cite{li2022trustworthy}. Specifically, we sample a subset using a specific decay distribution $P_{d}(y)$, such as an exponential distribution~\cite{cui2019class} or a Pareto distribution~\cite{liu2019large}, as follows:
\begin{equation}
    P^{'}(\{\boldsymbol{X}^{v}\}^V_{v=1} | y=k) 
    = P_{d}\{y=k\}P(\{\boldsymbol{X}^{v}\}^V_{v=1} | y=k).
\end{equation}
where samples from the $k$-th class are randomly selected with probability $P_{d}\{y=k\}$ to construct a class imbalance multi-view classification input. In our experiment, we employ an exponential decay rate $\eta=0.3$ to generate the imbalanced training set, where the number of samples decreases as the class label increases. \cref{fig:Number of samples} shows the sample distribution of traning and test sets using our data generation strategy on the HandWritten dataset. It is clear that the the training set follows a long-tail distribution, with tail classes containing significantly fewer samples than head classes. For single-view methods, we report the results from the best-performing view. All results are obtained by averaging 10 trials.

\begin{figure}[t]
  \centering
   \includegraphics[width=0.7\linewidth]{img/Number of samples.drawio.pdf}
   \caption{Sample distribution of training and test sets on HandWritten dataset.}
   \label{fig:Number of samples}
\end{figure}

\subsection{Experiment Results}

\textbf{Accuracy Comparison.} \Cref{table:classficiation} presents the comparison results of various methods on standard test sets. It is evident that our proposed TMLC method significantly outperforms all baseline methods on the class-balanced test set, particularly on the PIE, NUS-WIDE, and Animal datasets, where it achieves performance improvements exceeding 5\%. We attribute this enhancement primarily to our uncertainty-based sample generation scheme, which ensures that the generated pseudo-samples more closely approximate the true sample distribution. These pseudo-samples effectively mitigate the class imbalance issue in multi-view data, thereby improving the model's classification accuracy. To further validate the effectiveness of the generated pseudo-samples, we conduct a comparative experiment by excluding the pseudo-sample generation module, resulting in a variant labeled as Ours-v1. The results show that Ours-v1 performs worse than the complete model across all tested datasets, demonstrating that the uncertainty-based sample generation scheme plays a crucial role in enhancing the network's classification performance.



\begin{table*}[h]
\centering
\small
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{Methods} & \multicolumn{6}{c}{Datasets} \\ 
% \cline{2-7}   
& HandWritten & PIE & Caltech101 & NUS-WIDE & Scene15 & Animal \\ \hline
TLC & 84.20$\pm$1.05 & 36.32$\pm$0.67 & 79.04$\pm$1.22 & 19.00$\pm$0.61 & 42.54$\pm$1.30 & 16.54$\pm$0.10 \\
H2T & 90.13$\pm$0.12 & 31.54$\pm$0.61 & 83.12$\pm$0.22 & 17.97$\pm$0.33 & 38.59$\pm$0.25 & 15.84$\pm$0.10 \\
TMC & 92.65$\pm$0.28 & 46.18$\pm$0.92 & 84.91$\pm$0.21 & 22.44$\pm$0.39 & 32.22$\pm$0.50 & 24.23$\pm$0.12 \\
ECML & 91.48$\pm$0.34 & \underline{47.28$\pm$0.74} & 82.87$\pm$0.56 & 22.35$\pm$0.27 & 41.31$\pm$0.71 & \underline{24.31$\pm$0.08} \\
DUA-Nets & 91.53$\pm$1.86 & 8.96$\pm$1.08 & 77.60$\pm$2.00 & 20.45$\pm$1.72 & 36.72$\pm$1.10 & 14.89$\pm$0.65 \\
DCP  & \underline{93.48$\pm$1.33} & 4.56$\pm$0.64 & \underline{86.54$\pm$1.15} & \underline{29.04$\pm$2.21} & \underline{53.56$\pm$1.22} & 18.77$\pm$0.63 \\ 
UIMC  & 91.35$\pm$0.46 & 45.88$\pm$1.51 & 79.58$\pm$0.74 & 20.98$\pm$0.80 & 48.02$\pm$0.38 & 20.90$\pm$0.41 \\ 
DMVLS   & 81.28$\pm$1.05 & 11.62$\pm$1.18 & 72.03$\pm$1.29 & 21.48$\pm$1.19 & 30.19$\pm$0.88 & 18.63$\pm$0.81 \\ 
\cline{1-7}
Ours-v1  & 93.40$\pm$0.28 & 48.38$\pm$1.03 & 83.76$\pm$0.48 & 26.31$\pm$0.19 & 45.20$\pm$0.41 & 24.34$\pm$0.06 \\ 
Ours   & \textbf{96.25$\pm$0.32} & \textbf{62.43$\pm$0.70} & \textbf{89.48$\pm$0.24} & \textbf{38.96$\pm$0.37} & \textbf{58.57$\pm$0.37} & \textbf{31.35$\pm$0.20} \\ 
\hline
\end{tabular}
\caption{Accuracy (\%) on class-balanced test sets. The best results are highlighted in bold, while the second-best are underlined.}
\label{table:classficiation}
\end{table*}

\textbf{Performance for Conflictive Noise.} To validate the superiority of the proposed group consensus opinion aggregation mechanism, we conduct experiments by introducing conflictive noise into the test data \cite{xu2024reliable}. We compare our approach with ECML, a state-of-the-art (SOTA) baseline for handling conflictive instances. \Cref{table:conflict} summarizes the comparison results on six datasets under both normal and conflict noise conditions. The results demonstrate that, in both scenarios, the group consensus opinion aggregation mechanism generally outperforms ECML. Specifically, on the NUS-WIDE dataset, our method achieves performance improvements of 5.5\% and 5.13\% in normal and conflict noise settings, respectively. These findings highlight the effectiveness of our proposed group consensus opinion aggregation in enhancing the aggregation of multi-view opinions, thereby leading to more reliable classification results.

\begin{table}[h]
\centering
\small
\begin{tabular}{c|c|cc}
\hline
\multirow{2}{*}{Datasets} & \multirow{2}{*}{Test sets} & \multicolumn{2}{c}{Methods} \\ \cline{3-4}
&  & ECML & Ours  \\ \hline
\multirow{2}{*}{HandWritten} & Normal & 97.00 & \textbf{97.50}  \\ \cline{2-4}
 & Conflictive & 92.69  & \textbf{94.80}  \\ \hline
\multirow{2}{*}{PIE} & Normal & 94.85 & \textbf{95.59}  \\ \cline{2-4}
 & Conflictive & 81.62  & \textbf{83.67}  \\ \hline
\multirow{2}{*}{Caltech101} & Normal & \textbf{93.88} & 93.08  \\ \cline{2-4}
 & Conflictive & 90.53  & \textbf{90.99}  \\ \hline
\multirow{2}{*}{NUS-WIDE} & Normal & 40.54 & \textbf{46.04}  \\ \cline{2-4}
 & Conflictive & 37.04  & \textbf{42.17}  \\ \hline
\multirow{2}{*}{Scene15} & Normal & 70.12 & \textbf{71.57}  \\ \cline{2-4}
 & Conflictive & 61.50  & \textbf{62.74}  \\ \hline
\multirow{2}{*}{Animal} & Normal & 58.31 & \textbf{59.48}  \\ \cline{2-4}
 & Conflictive & 49.39  & \textbf{51.05}  \\ \hline
\end{tabular}
\caption{Accuracy (\%) on normal and conflictive test sets. The best results are highlighted in bold.}
\label{table:conflict}
\end{table}

\textbf{Uncertainty Estimation.} In order to assess the uncertainty of the model predictions, we visualize the distribution of both in-distribution and out-of-distribution samples. Specifically, the original samples and the samples with added Gaussian noise are considered as in-distribution and out-of-distribution samples, respectively. The experiment is conducted on the PIE dataset, where Gaussian noise with different standard deviations $(\sigma = 0.1, \sigma = 1, \text{and } \sigma = 10)$ is added to the test samples, as shown in \cref{fig:Uncertainty}. The results indicate that as the noise intensity increases, the uncertainty of the data also increases, and the distribution curve of the out-of-distribution samples deviates more significantly from that of the in-distribution samples. This suggests that the proposed group consensus opinion aggregation strategy effectively captures the uncertainty, thereby improving the overall reliability of the model.

\begin{figure}[t]
  \centering
   \includegraphics[width=0.7\linewidth]{img/KDE.drawio.pdf}
   \caption{Density of overall uncertainty on the PIE
   dataset.}
   \label{fig:Uncertainty}
\end{figure}

\textbf{Joint Evidence Visualization.} To validate the rationale of the newly defined evidence-based distance metric in the uncertainty-based sample generation scheme, \cref{fig:evidence visual} visualizes the evidence obtained from the aggregation mechanism on six multi-view datasets. Our observations are as follows: (1) Evidence points belonging to the same class are clustered closely together, while those from different classes are distinctly separated. This demonstrates that the evidence-based distance effectively captures class-specific information and accurately constructs neighbor relationships. (2) As the degree of class imbalance increases, the limited number of training samples results in reduced evidence and heightened uncertainty. Consequently, these classes tend to form neighbor relationships with other challenging-to-classify classes.

\begin{figure*}[t]
  \centering
   \includegraphics[width=0.8\linewidth]{img/evidence_visual.drawio.pdf}
   \caption{Joint evidence visualization on different datasets.}
   \label{fig:evidence visual}
\end{figure*}

\textbf{Performance Evaluation under Different Decay Rates.} To demonstrate the superiority of our TMLC model in noisy environments, we conduct experiments by introducing varying levels of decay rates into the training data, with the decay rate ranging over $[0, 0.05, 0.10, 0.15, 0.20, 0.25, 0.30]$. \Cref{fig:Different Decay Rates} illustrates the performance comparison of all methods on the PIE dataset under different decay rates. It is evident that, compared to the baseline methods, our TMLC model consistently outperforms them across all tested datasets at each decay rate, further validating the effectiveness of the proposed pseudo-data generation scheme. Furthermore, to verify the superiority of the weight calculation scheme, we replace the designed weight mechanism with random weights, resulting in a variant labeled as Ours-v2. The experimental results confirm that the uncertainty-induced weight scheme more effectively integrates neighboring samples from different views, thereby generating synthetic samples that better align with the characteristics of the minority class.

\begin{figure}[t]
  \centering
   \includegraphics[width=0.7\linewidth]{img/Different Decay Rates.drawio.pdf}
   \caption{Performance comparison on PIE datasets with varying decay rates.}
   \label{fig:Different Decay Rates}
\end{figure}

\textbf{Parameter Selection.} Since the model requires a predefined number of neighbors, $R$, we conduct experiments with different values of $R = [1, 2, 3, 5, 7, 9]$ to investigate its impact. As shown in \cref{fig:R_PIE}, as the number of neighbors increases, the generated multi-view pseudo-samples incorporate more relevant sample information, which enhances the diversity of the samples and improves the classification performance. However, beyond a certain value of $R$, the classification performance approaches stability. This is because the sample knowledge has already been sufficiently integrated, and further increasing the number of neighbors does not provide additional useful information, resulting in negligible improvements in classification performance.

\begin{figure}[t]
  \centering
   \includegraphics[width=0.7\linewidth]{img/R_PIE.drawio.pdf}
   \caption{Accuracy comparison with respect to $R$.}
   \label{fig:R_PIE}
\end{figure}

==> sec/5_conclusion.tex <==
\section{Conclusion}

In this paper, we propose a trusted multi-view learning framework for long-tailed classification, namely TMLC . TMLC makes two significant contributions. First, inspired by Social Identity Theory, we design a group consensus opinion aggregation mechanism that aligns decision-making with the collective judgment of the majority. Second, we develop an innovative pseudo-data generation strategy that integrates a novel evidence-based distance metric and an uncertainty-guided module to produce high-quality synthetic samples. Extensive experiments demonstrate the superior performance of TMLC.

==> sec/6_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{iccv.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/7_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/8_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
